MathVista: Evaluating Mathematical Reasoning of Foundation Models in Visual Contexts

Large Language Models (LLMs) and Large Multimodal Models (LMMs) exhibit impressive problem-solving skills in many tasks and domains, but their ability in mathematical reasoning in visual contexts has not been systematically studied. To bridge this gap, we present MathVista, a benchmark designed to combine challenges from diverse mathematical and visual tasks. It consists of 6,141 examples, derived from 28 existing multimodal datasets involving mathematics and 3 newly created datasets (i.e., IQTest, FunctionQA, and PaperQA). Completing these tasks requires fine-grained, deep visual understanding and compositional reasoning, which all state-of-the-art foundation models find challenging. With MathVista, we have conducted a comprehensive, quantitative evaluation of 12 prominent foundation models. The best-performing GPT-4V model achieves an overall accuracy of 49.9%, substantially outperforming Bard, the second-best performer, by 15.1%. Our in-depth analysis reveals that the superiority of GPT-4V is mainly attributed to its enhanced visual perception and mathematical reasoning. However, GPT-4V still falls short of human performance by 10.4%, as it often struggles to understand complex figures and perform rigorous reasoning. This significant gap underscores the critical role that MathVista will play in the development of general-purpose AI agents capable of tackling mathematically intensive and visually rich real-world tasks. We further explore the new ability of self-verification, the application of self-consistency, and the interactive chatbot capabilities of GPT-4V, highlighting its promising potential for future research. The project is available at https://mathvista.github.io/.

==> backups/introduction_old_v1.tex <==


\section{Introduction}
\label{sec:introduction}




A long-standing goal of AI is to create general-purpose assistants that can tackle diverse unseen tasks. The recent revolution in Large Language Models (LLMs) such as ChatGPT~\citep{openai2022chatgpt}, Claude~\citep{claude2}, and GPT-4~\citep{openai2023gpt4} has given rise to potent foundation models, trained on vast text corpora and fine-tuned on high-quality instruction data. Concurrently, the fusion of vision and language has propelled the development of Large Multimodal Models (LMMs) like LLaMA-Adapter V2~\citep{gao2023llamaadapterv2}, LLaVA~\citep{liu2023llava}, Bard~\citep{google2023bard}, and the latest GPT-4V~\citep{openai2023gpt4v}, designed to respond to human queries within visual contexts. Despite these remarkable advancements, a significant gap persists in our understanding of their mathematical reasoning capabilities within visual scenarios due to the lack of systematic evaluations.
% instruction-response data with human alignments
% evaluating these models on a set of diverse tasks demanding rigorous mathematical reasoning within visual scenarios. \hb{can say: a significant gap persists in our understanding of their math reasoning capabilities due to the lack of any systematic eval}
% \hb{there should a closing line to this para so the reader understands the broad problem our paper addresses}
% \hb{worth mentioning gpt-4-v as well}

% While both LLMs and their multimodal counterparts excel at addressing general domains and facilitating simple conversations, they fall short in building truly general-purpose assistants, especially for tasks where rigorous logical reasoning is required \hb{cut this line}. Among these tasks,\hb{can cut among these tasks,} \hb{Just start by saying Math reasoning stands out...} 
Mathematical reasoning stands out as particularly challenging due to its demand for rigorous reasoning and problem-solving abilities, which necessitate domain-specific knowledge and multistep abstract reasoning. Agents with strong mathematical reasoning capabilities have various practical applications, such as solving complex problems in educational disciplines~\citep{seo2015solving,wang2017deep}, helping analysts answer logical queries about statistical data~\citep{wu2023bloomberggpt,yang2023fingpt}, and assisting in theorem proving and scientific discovery in advanced research fields~\citep{taylor2022galactica,dong2023large}. 

Datasets such as GSM-8K~\citep{cobbe2021training} have been curated to assess the ability of LLMs to perform mathematical reasoning on problems presented in natural language. However, many mathematical problems are inherently grounded in a visual modality, including abstract scenes, geometry diagrams, and figures. These problems have been the focus of some recent studies \citep{lu2021inter,dahlgren2022clevr,masry2022chartqa}. Notably, these datasets prioritize the evaluation of models in specific tasks (e.g., math word problems) or visual contexts (e.g., bar charts). Additionally, there are general-purpose vision-language datasets, such as VQA 2.0~\citep{goyal2017making} and OK-VQA~\citep{schwenk2022okvqa}, which also feature instances requiring mathematical reasoning over photos of everyday scenes (e.g., inferring the age gap between two famous people). Recently, various approaches have been developed to augment the LLMs' capabilities in visual contexts, either by equipping them with external tools~\citep{lu2023chameleon} or through end-to-end training with visual encoders~\citep{gao2023llamaadapterv2}. To this end, novel datasets are essential to bridge the gap, and systematic benchmarking becomes crucial to probe the capabilities of foundational models.

% Considering this backdrop of advancements in combining visual comprehension with mathematical reasoning in AI models, novel datasets and systematic benchmarking become essential to probe their capabilities in the

% for the evolution of AI models

% ---an area we aim to contribute by proposing a consolidated benchmark. 

% and extend the diversity of contexts by integrating photos of everyday scenes. 
% like Geometry3K~\citep{lu2021inter}, ChartQA~\citep{masry2022chartqa}, FigureQA~\citep{kahou2017figureqa}, and CLEVR-Math~\citep{dahlgren2022clevr}

% We believe key considerations for this endeavor should include diversity in visual contexts, reasoning types, grade levels, and a range of tasks. Consequently, it is pertinent to provide a more thorough assessment of models' capacities in real-world, visually-rich problem-solving scenarios.

% , which are absent in conventional MathQA datasets, thus necessitating different types of reasoning skills
% over the zero-shot \hb{we also test beyond 0shot abilties: something like foundation models without any task-specific finetuning.} abilities of foundational models.
% \hb{what is special in these datasets that is missing in regular mathqa datasets?}. \hb{this line on tool-augmented models does not fit here.} 
% Given this landscape \hb{what landscape?},
% systematic benchmarking becomes essential for the evolution of AI models---a gap we are eager to address \hb{very generic line which does not address anything}.
% benchmark foundational models for mathematical reasoning within visual contexts. 

% \textbf{Paragraph 3}
% \begin{enumerate}
%     \item We propose MathVista, ..
%     \item Talk about how it is created
%     \item Talk about data analysis
% \end{enumerate}

% \chunyl{the shortname is great, but I can not see how it can be made from the full name} \hb{i don't think we need to show that MathVista is a short name for a long name -- can just unbold Math and Vis from the previous line}
% Can we also mention that we created 3 new datasets? Otherwise this sentence might make reader think our Benchmark is merely a collection of existing ones .
In this work, we propose \dataset, a consolidated \underline{\textbf{Math}}ematical reasoning benchmark within \underline{\textbf{Vis}}ual contexts. \dataset consists of three new datasets we created: IQTest, FunctionQA, and PaperQA, together with 9 math-targeted question answering (MathQA) datasets and 19 visual question answering (VQA) datasets in the literature. The inclusion of existing datasets significantly enriches the diversity and complexity of visual perception and mathematical reasoning challenges within our benchmark. As illustrated in Figure~\ref{fig:our_new_3_datasets}, the three new data sets that we collected address the gap in existing datasets and are tailored to evaluate mathematical reasoning skills in specific visual contexts of puzzle test figures, functional plots, and academic paper figures, respectively.  We focus on both multiple-choice questions (e.g., choose among four options) and free-form questions with numeric answers (e.g., answer in integer or decimal), aiming for deterministic evaluation metrics. \dataset encompasses 6,141 examples, with 736 of them being newly annotated (see Table~\ref{tab:statistics} for key statistics). To facilitate fine-grained metrics, examples are further enriched with extensive metadata---covering question, answer, task, grade level, visual context, and reasoning skills. More details on data collection and analysis can be found in \S \ref{sec:dataset}, \S \ref{sec:collection_guideline}, and \S \ref{app:collection_details}.

\begin{figure}[t!]
  \centering
  \vspace{-3mm}
  \includegraphics[width=1.0\textwidth]{figs/tease_scores.pdf}
  \vspace{-3mm}
  \caption{Accuracy scores of one leading LLM (PoT GPT-4) and five primary LMMs on our proposed \dataset across mathematical reasoning and visual context types. Scores are adjusted by subtracting the random chance score and normalized to a range of $0-100$. PoT refers to program-of-thought prompting, and PoT GPT-4 is a textual LLM augmented with the caption and OCR text.}
  \vspace{-3mm}
\label{fig:tease_scores}
\end{figure}

% \hb{mention the section number where you provide more details}.

% are sourced from 9 math-targeted question answering (MathQA) datasets and 19 visual question answering (VQA) datasets in the literature. The incorporation of 19 VQA datasets alongside math-targeted datasets is motivated by our objective to explore a wide array of visual contexts, thereby enriching the diversity and complexity of mathematical reasoning challenges encompassed within our benchmark. We focus on both multi-choice questions (e.g., choose among four options) and free-form questions with numeric answers (e.g., answer in integer or decimal), aiming for deterministic evaluation metrics. To discern VQA questions that require mathematical reasoning, we use heuristic rules such as identifying the presence of quantitative terms and numerical entities within the question and answer pairs to retain qualified samples. Annotators then manually remove any false positives. To address the lack of datasets catering to specific visual contexts, we annotate and collect three additional new source datasets: IQTest, FunctionQA, and PaperQA, tailored to evaluate mathematical reasoning skills in the contexts of puzzle test figures, functional plots, and academic paper figures, respectively (refer to Figure~\ref{fig:our_new_3_datasets}). 

% We split the examples into two subsets: \textit{minitest} intended for model development or for those with restricted computing resources, and \textit{test} as standard evaluation. For the latter, we will not disclose the answers publicly and employ an online platform with automated evaluations to prevent data contamination.

% ---achieved through automated labeling followed by human refinement. 

\begin{figure}[th!]
  \centering
  \vspace{-3mm}
  \includegraphics[width=1.0\textwidth]{figs/our_new_3_datasets.pdf}
  \vspace{-4mm}
  \caption{Examples of our newly annotated datasets: IQTest, FunctionQA, and PaperQA.}
  \vspace{-3mm}
\label{fig:our_new_3_datasets}
\end{figure}


 % pertaining to mathematical reasoning in the existing literature
% \hb{which gaps? there is no gap being talked about anywhere before} 
% (\hb{unclear --> what kind of heuristic rules? }) to retain samples with quantitative words in the questions and numerals in the answers.
% \hb{why do you want to look at the 19 VQA datasets when math-targeted already exist? talk about the diversity in the visual contexts}  
 % \hb{``e'' of the highlighted ``te'' is not in MathVista}.
% Each source dataset is limited to up to 400 examples to ensure thorough evaluation \hb{how does 400 examples ensures thorough evaluation. i think you can remove this line from the introduction}. 

% \textbf{Paragraph 4}
% \begin{enumerate}
%     \item Results
%     \item Analysis
% \end{enumerate}

We conduct comprehensive experiments to evaluate the reasoning abilities of a set of foundation models on \dataset, including three LLMs, seven open-source LMMs, and one proprietary LMM. For LLMs, we study zero-shot and few-shot settings using two prompting strategies, chain-of-thought (CoT) \citep{wei2022chain} and program-of-thought (PoT) \citep{chen2022program}, as well as their augmented variants with image caption and OCR text from off-the-shelf visual models to explore their potential on \dataset. We design an LLM-based answer extractor to derive the final short answers from generated free-form responses, allowing consistent and scalable evaluations. 

% Instead of human evaluation or manually designed rules in existing works~\citep{lu2022learn}, \hb{start the sentence directly from here}
 
The results show that the state-of-the-art (SOTA) LLM without visual tool augmentations, CoT GPT-4, achieves an overall accuracy score of 29.2\%, while the SOTA LMM, Multimodal Bard, achieves 34.8\% (\S \ref{sec:results}). There is substantial room for improvement, with human performance reaching 60.3\%. By augmenting with Bard image captions and detected OCR text, PoT GPT-4 obtains 33.9\%, comparable to Multimodal Bard (\S \ref{fine_grained_results}). The results of the leading model are highlighted in Figure ~\ref{fig:tease_scores}. Further analysis reveals that failure reasons include incorrect calculations and hallucinations caused by visual perception and textual reasoning (\S \ref{app:qualitative_analysis}). These results suggest two future directions: (1) proposing general-purpose LMMs with enhanced visual perception and mathematical reasoning; (2) developing augmented LLMs powered by external tools to improve visual perception and domain-specific reasoning abilities.

 % for future work
% , along with failure analysis, 
% the predominant reason for the wrong answers for Multimodal Bard is because of wrong or partially wrong explanations \hb{last few words are confusing, simplify}, caused by incorrect reasoning with hallucinations and wrong calculations 
% Random chance and frequent guesses are used as the baseline performance measures, along with a human performance study. 
% \textbf{Paragraph 1}
% \begin{enumerate}
%     \item long standing aim of AI is to build general purpose assistants that can solve diverse unseen tasks. Among these tasks, mathematical reasoning is quite challenging since it requires the problem solving abilities which include multi-step logical reasoning, domain-specific knowledge.
%     \item Agents with strong mathematical reasoning capabilities have many practical applications such as aiding analysts in answering logical questions about their data, solving complex geometrical problems in scientific domains and pedagogy. (Add citations)
%     \item Recent revolution in LLMs has created very powerful foundation models that are trained on large corpora of text, and finetuned on high-quality of instruction+response data with human alignment aka ChatGPT, GPT-4. 
%     \item On the multimodal side (language + vision), there has been a surge of large multimodal models - Multimodal Bard, Llava, ..etc. that can answer human queries posed as questions or imperative tasks. 
% \end{enumerate}
% \chenghao{Probably want to first say both LLMs and their multi-modality counterparts are good at general domain/simple conversations Then, argue it is not enough for building general-purpose assistants, especially for cases where rigorous logic and math reasoning is required (examples and applications listed). 
% Maybe also layout the prominent approaches for extending LLMs to handle visual contexts: 1) augmented LLMs, 2) end-to-end training with visual encoders.
% then say, systematical benchmarking is critical for the development of AI models, we want to fill this gap. then move to short review of math-focused datasets for LLMs and multi-modality ones and why they are not sufficient. Probably, we also want to say sth about what we think are desiderata of math-reasoning with visual contexts, e.g., diversity in visual contexts, reasoning types, difficulty levels, ...}

% \textbf{Paragraph 2}
% \begin{enumerate}
%     \item Talk about datasets such as GSM8K, MathQA that assess their ability to perform math reasoning on problems expressed in natural language. These works suggest that ...
%     \item However, many mathematical problems are naturally grounded in visual modality such as geometrical problems, chart reasoning, math reasoning in natural scenes. (cite Unigeo, ChartQA, PlotQA, Clevr-Math). However, these datasets evaluate task-specific models rather than zero-shot abilities of the foundation models.
%     \item In addition, there are many general purpose vision-text datasets such as VQA, OKVQA which contain instances that require mathematical reasoning. 
%     \item To this end, it is pertinent to benchmark the foundation models for mathematical reasoning in visual contexts. 
% \end{enumerate}

% \hb{it is fine to just say Foundation Models in the title but the main text should be clear.}
% \pan{need clarification here}


% \include{tables/our_new_3_dataset}




==> backups/introduction_old_v2.tex <==

\section{Introduction}
\label{sec:introduction}


% A long-standing goal of AI is to create general-purpose assistants that can tackle diverse unseen tasks. The recent revolution in Large Language Models (LLMs) such as ChatGPT~\citep{openai2022chatgpt}, Claude~\citep{claude2}, and GPT-4~\citep{openai2023gpt4} has given rise to potent foundation models, trained on vast text corpora and fine-tuned on high-quality instruction data. Concurrently, the fusion of vision and language has propelled the development of Large Multimodal Models (LMMs) like LLaMA-Adapter V2~\citep{gao2023llamaadapterv2}, LLaVA~\citep{liu2023llava}, Bard~\citep{google2023bard}, and the latest GPT-4V~\citep{openai2023gpt4v}, designed to respond to human queries within visual contexts. 

% Hana: 1. The first paragraph is just naming a lot of llms and lmms... Summarize that in 1-2 lines. ; Just write a sentence that we have witnessed great progress in foundation models in text (citations or just bring one name) and vision-language models (eg... 1-2 names). it is important to evaluate math reasoning skills.

A long-standing goal of AI is to create general-purpose assistants that can tackle diverse unseen tasks. We have witnessed great progress in foundation models in text such as ChatGPT \citep{openai2022chatgpt,openai2023gpt4} and in vision-language models such as Bard~\citep{google2023bard} and GPT-4V~\citep{openai2023gpt4v}. Despite these advances, a significant gap persists in our understanding of their mathematical reasoning capabilities within visual scenarios due to the lack of systematic evaluations.

\kw{Like my comments in abstract, there is a logical gap between saying the existing model performs well to the evaluation of visual math reasoning skill.}

\kw{If you want to start intro with this flow. You may first argue that there are several benchmark and studies to investigate the math reasoning skill and visual reocgnizaiton skill of models. However, the combined of these two raises additional challenges. Then emphasize why visual math reasoning skill is essential and should be evaluated.}

\kw{But I think you may also just remove the first paragraph and just stariting with discussing math reasoning skill and treat your paper as an extension to the existing benchmark by augmenting visual context. }

Mathematical reasoning is challenging due to its demand for rigorous reasoning and problem-solving abilities, requiring domain-specific knowledge and multistep reasoning. Agents with strong mathematical reasoning capabilities have various applications, such as solving complex problems in educational disciplines~\citep{seo2015solving,wang2017deep}, helping analysts with logical queries about statistical data~\citep{wu2023bloomberggpt,yang2023fingpt}, and assisting in theorem proving and scientific discovery in advanced research fields~\citep{taylor2022galactica,dong2023large}. 



% Datasets such as GSM-8K~\citep{cobbe2021training} have been curated to assess the ability of LLMs to perform mathematical reasoning on problems presented in natural language. However, many mathematical problems are inherently grounded in a visual modality, including abstract scenes, geometry diagrams, and figures. These problems have been the focus of some recent studies \citep{lu2021inter,dahlgren2022clevr,masry2022chartqa}. Notably, these datasets prioritize the evaluation of models in specific tasks (e.g., math word problems) or visual contexts (e.g., bar charts). Additionally, there are general-purpose vision-language datasets, such as VQA 2.0~\citep{goyal2017making} and OK-VQA~\citep{schwenk2022okvqa}, which also feature instances requiring mathematical reasoning over photos of everyday scenes (e.g., inferring the age gap between two famous people). Recently, various approaches have been developed to augment the LLMs' capabilities in visual contexts, either by equipping them with external tools~\citep{lu2023chameleon} or through end-to-end training with visual encoders~\citep{gao2023llamaadapterv2}. To this end, novel datasets are essential to bridge the gap, and systematic benchmarking becomes crucial to probe the capabilities of foundational models.

% Hana: 2. Acknowledge that there are many datasets in text; but we need language/vision datasets. There are some in language/vision, but either focused on specific domains or part of general VQA datasets, but a comprehensive study of language/vision QA is missing. 


Numerous datasets such as GSM-8K~\citep{cobbe2021training} have been curated to assess the mathematical reasoning abilities of Large Language Models (LLMs) through problems presented purely in text. However, many mathematical problems are inherently grounded in a visual modality, including geometry diagrams and scientific figures. While some datasets \citep{lu2021inter,dahlgren2022clevr,masry2022chartqa} have explored mathematical reasoning in vision-language settings, they tend to either emphasize specific tasks, like math word problems, or particular visual contexts, such as geometry problems or bar charts. General-purpose visual question answering (VQA) datasets only contain a small portion of questions that require mathematical reasoning, leaving a comprehensive study of vision-language reasoning within a mathematical framework largely unexplored. Recent endeavors have aimed to bolster the mathematical and scientific reasoning capabilities in visual contexts by augmenting models with external tools~\citep{lu2023chameleon}. To this end, the creation of novel datasets and systematic benchmarking becomes crucial to probe the capabilities of foundational models in tackling mathematical reasoning challenges within visual scenarios.

\kw{``However, many mathematical problems are": I feel this argument is a bit weak -- it doesn't really motivate why we want to verify model's math reasoning ability with visual context.}

\kw{I think we may motivate by saying when we assessing a kid's math and reasoning skills, beside arithmetic calculation, we often design problems that invovles visual contexts. (see if you can find some reference in education?) 
}

% In this work, we propose \dataset, a consolidated \underline{\textbf{Math}}ematical reasoning benchmark within \underline{\textbf{Vis}}ual contexts. \dataset consists of three new datasets we created: IQTest, FunctionQA, and PaperQA, together with 9 math-targeted question answering (MathQA) datasets and 19 visual question answering (VQA) datasets in the literature. The inclusion of existing datasets significantly enriches the diversity and complexity of visual perception and mathematical reasoning challenges within our benchmark. As illustrated in Figure~\ref{fig:our_new_3_datasets}, the three new data sets that we collected address the gap in existing datasets and are tailored to evaluate mathematical reasoning skills in specific visual contexts of puzzle test figures, functional plots, and academic paper figures, respectively.  We focus on both multiple-choice questions (e.g., choose among four options) and free-form questions with numeric answers (e.g., answer in integer or decimal), aiming for deterministic evaluation metrics. \dataset encompasses 6,141 examples, with 736 of them being newly annotated (see Table~\ref{tab:statistics} for key statistics). To facilitate fine-grained metrics, examples are further enriched with extensive metadata---covering question, answer, task, grade level, visual context, and reasoning skills. More details on data collection and analysis can be found in \S \ref{sec:dataset}, \S \ref{sec:collection_guideline}, and \S \ref{app:collection_details}.

% Hana: 4. You introduce mathvista; a taxonomy; and then three new datasets to fill the gap. MathVista consists of xxx datasets, and xxx instances. 

In this paper, we introduce \dataset, a consolidated \underline{\textbf{Math}}ematical reasoning benchmark within \underline{\textbf{Vis}}ual contexts. We propose a taxonomy as the guideline for constructing \dataset: (1) we identify seven mathematical reasoning types: \textit{algebraic reasoning}, \textit{arithmetic reasoning}, \textit{geometry reasoning}, \textit{logical reasoning}, \textit{numeric common sense}, \textit{scientific reasoning}, and \textit{statistical reasoning}; (2) we focus on five primary tasks: \textit{figure question answering} (FQA), \textit{geometry problem solving} (GPS), \textit{math word problem} (MWP), \textit{textbook question answering} (TQA), and \textit{visual question answering} (VQA); and (3) we aim at encompassing a diverse array of visual contexts, including natural images, geometry diagrams, abstract scenes, synthetic scenes, as well as various figures, charts, and plots. We create three new datasets, IQTest, FunctionQA, and PaperQA, which address the missing mathematical and visual domains and are tailored to evaluate logical reasoning on puzzle test figures, algebraic reasoning over functional plots, and scientific reasoning with academic paper figures, respectively. \dataset also incorporates 9 math-targeted question answering (MathQA) datasets and 19 VQA datasets (after filtration) from the literature, which significantly enrich the diversity and complexity of visual perception and mathematical reasoning challenges within our benchmark. \dataset consists of 6,141 examples, with 736 of them being newly annotated (see Table~\ref{tab:statistics} for key statistics). To facilitate fine-grained metrics, examples are further enriched with extensive metadata---covering question, answer, task, grade level, visual context, and reasoning skills. More details on data collection and analysis can be found in \S \ref{sec:dataset}, \S \ref{sec:collection_guideline}, and \S \ref{app:collection_details}.


\begin{figure}[t!]
  \centering
  \vspace{-3mm}
  \includegraphics[width=1.0\textwidth]{figs/tease_scores.pdf}
  \vspace{-3mm}
  \caption{Accuracy scores of one leading LLM (PoT GPT-4) and five primary LMMs on our proposed \dataset across mathematical reasoning and visual context types. Scores are adjusted by subtracting the random chance score and normalized to a range of $0-100$. PoT refers to program-of-thought prompting, and PoT GPT-4 is a textual LLM augmented with the caption and OCR text.}
  \vspace{-2mm}
\label{fig:tease_scores}
\end{figure}

We conduct comprehensive experiments on \dataset to evaluate the reasoning abilities of 11 foundation models known for their leading performance in mathematical reasoning and multimodal reasoning. This ensemble includes three LLMs, seven open-source LMMs, and one proprietary LMM. For LLMs, we study zero-shot and few-shot settings using two prompting strategies, chain-of-thought (CoT) \citep{wei2022chain} and program-of-thought (PoT) \citep{chen2022program}, as well as their augmented variants with image caption and OCR text from off-the-shelf visual models to explore their potential on \dataset. We design an LLM-based answer extractor to derive the final short answers from generated free-form responses, allowing consistent and scalable evaluations. Additionally, we established a human performance baseline by engaging human annotators who passed the qualification examples and possessed a high school or higher degree. Given that \dataset features advanced topics like college curricula and scientific reasoning, it proves to be a challenging benchmark, with human performance reaching only 60.3\% accuracy.

% \kw{this may raise a question -- human reaching only 60\% because of what? it becauses the problem is hard and human also lacks of skill to do so or because the annotations are bad so there are noise. If it's former, what is the level of expertise? We need to be a bit more specific here. }

The results show that CoT GPT-4, the best performing LLM without visual tool augmentations, achieves an overall accuracy of 29.2\%, while the best performing LMM, Multimodal Bard, achieves 34.8\% (\S \ref{sec:results}). Notably, Multimodal Bard achieves only 58\% of human performance (34.8\% vs 60.3\%), indicating substantial room for further improvement. By augmenting with Bard image captions and detected OCR text, PoT GPT-4 obtains 33.9\%, comparable to Multimodal Bard (\S \ref{fine_grained_results}). The results of the primary model are highlighted in Figure ~\ref{fig:tease_scores}. Further analysis reveals that failure reasons include incorrect calculations and hallucinations caused by visual perception and textual reasoning (\S \ref{app:qualitative_analysis}). These results suggest two future directions: (1) proposing general-purpose LMMs with enhanced visual perception and mathematical reasoning; (2) developing augmented LLMs powered by external tools to improve visual perception and domain-specific reasoning abilities.


\begin{figure}[t!]
  \centering
  \vspace{-3mm}
  \includegraphics[width=1.0\textwidth]{figs/our_new_3_datasets.pdf}
  \vspace{-5mm}
  \caption{Examples of our newly annotated datasets: IQTest, FunctionQA, and PaperQA.}
  \vspace{-2mm}
\label{fig:our_new_3_datasets}
\end{figure}



==> backups/main_results_v1.tex <==

\begin{table*}[t!]
\centering
 \small
 \renewcommand\tabcolsep{3.0pt} % column space
 \renewcommand\arraystretch{1.0} % row space
 \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|c|c|cc|ccccccc}
    \toprule
    \header{Model} & Input & \header{ALL} & \header{MC} & \header{FF} & \header{ALG} & \header{ARI} & \header{GEO} & \header{LOG} & \header{NUM} & \header{SCI} & \header{STA}  \\ 
    \midrule
    \multicolumn{12}{l}{\hfill \textit{Heuristics  baselines}} \\
    \midrule
    % \rowcolor[rgb]{0.93,0.93,0.93} \multicolumn{11}{l}{\textit{Heuristic baselines}} \\
    Random guess & - & 17.9 & 33.1 & 0.0 & 21.7 & 14.7 & 20.1 & 13.5 & 8.3 & 17.2 & 16.3 \\
    Frequent guess & - & 26.3 & 39.6 & 10.7 & 33.1 & 18.7 & 31.4 & 24.3 & 19.4 & 32.0 & 20.9 \\
    \midrule
    % \multicolumn{11}{l}{\hfill \text{Published results (Above)} $\blacktriangle$} \\
    \multicolumn{12}{l}{\hfill \textit{Large Language Models (LLMs)} } \\
    \midrule
    Zero-shot ChatGPT~\citeyearpar{openai2022chatgpt} & $Q$ only & 23.5 & 40.6 & 3.5 & 27.7 & 15.9 & 25.7 & \highclass{21.6} & 9.9 & 41.5 & \highclass{20.5} \\
    Zero-shot GPT-4~\citeyearpar{OpenAI2023GPT4TR} & $Q$ only & 26.1 & \highclass{46.7} & 2.0 & \highclass{33.6} & 17.4 & \highclass{35.6} & 16.2 & 9.2 & \highclass{45.8} & 19.5 \\
    Zero-shot Claude-2~\citeyearpar{claude2}& $Q$ only & \highclass{26.4} & 44.4 & \highclass{5.2} & 32.8 & \highclass{20.4} & 33.3 & 13.5 & \highclass{12.1} & 36.4 & \highclass{20.5} \\
    \midrule
    \multicolumn{12}{l}{\hfill \textit{Augmented Large Language Models (A-LLMs)} } \\
    \midrule
    2-shot CoT Claude-2~\citeyearpar{claude2} & $Q$, $I_c$, $I_t$ & 33.2 & 44.6 & \bestclass{19.8} & 31.0 & \bestclass{32.9 }& 31.0 & 16.2 & 17.4 & 50.8 & 37.2 \\
    2-shot CoT ChatGPT~\citeyearpar{openai2022chatgpt} & $Q$, $I_c$, $I_t$ & 33.2 & 46.1 & 18.0 & 32.4 & 32.3 & 33.0 & 16.2 & 17.4 & 54.9 & 36.2 \\
    2-shot CoT GPT-4~\citeyearpar{OpenAI2023GPT4TR} & $Q$, $I_c$, $I_t$ & 33.2 & \highclass{47.2} & 16.7 & 33.5 & 30.9 & 32.2 & 13.5 & 12.5 & \bestclass{58.2} & \bestclass{37.9} \\
    % \midrule
    2-shot PoT ChatGPT~\citeyearpar{openai2022chatgpt}& $Q$, $I_c$, $I_t$ & 26.8 & 38.5 & 13.0 & 27.8 & 26.1 & 28.0 & \highclass{18.9} & 13.2 & 33.6 & 29.9 \\
    2-shot PoT GPT-4~\citeyearpar{OpenAI2023GPT4TR} & $Q$, $I_c$, $I_t$ & \highclass{33.9} & 46.3 & 19.4 & \highclass{37.4} & 31.7 & \highclass{41.0} & \highclass{18.9} & \highclass{20.1} & 44.3 & \bestclass{37.9} \\
    \midrule
    \multicolumn{12}{l}{\hfill \textit{Vision-Language Models (VLMs)}} \\
    \midrule
    IDEFICS-9B-Instruct~\citeyearpar{laurencon2023obelics} & $Q$, $I$ & 19.8 & 32.2 & 5.2 & 22.1 & 15.0 & 19.8 & 18.9 & 9.9 & 24.6 & 18.1 \\
    mPLUG-Owl-LLaMA-7B ~\citeyearpar{ye2023mplug} & $Q$, $I$ & 22.2 & 35.4 & 6.7 & 23.6 & 19.2 & 23.9 & 13.5 & 12.7 & 26.3 & 21.4 \\
    miniGPT4-LLaMA-2-7B~\citeyearpar{zhu2023minigpt} & $Q$, $I$ & 23.1 & 35.4 & 8.7 & 28.1 & 21.0 & 24.7 & 16.2 & 16.7 & 25.4 & 17.9 \\
    LLaMA-Adapter-V2-7B~\citeyearpar{gao2023llamaadapterv2} & $Q$, $I$ & 23.9 & 37.2 & 8.3 & 26.3 & 20.4 & 24.3 & \bestclass{24.3} & 13.9 & 29.5 & 18.3 \\
    InstructBLIP-Vicuna-7B~\citeyearpar{instructblip} & $Q$, $I$  & 25.3 & 37.6 & 10.9 & 21.8 & 27.1 & 20.7 & 18.9 & \bestclass{20.4} & 33.0 & 23.1 \\
    LLaVA-LLaMA-2-13B~\citeyearpar{liu2023llava} & $Q$, $I$ & 26.1 & 38.9 & 11.1 & 27.3 & 20.1 & 28.8 & \bestclass{24.3} & 18.3 & 37.3 & 25.1 \\
    Multimodal Bard~\citeyearpar{google2023bard} & $Q$, $I$  & \bestclass{34.8} & \bestclass{48.7} & \highclass{18.5} & \bestclass{46.5} & \highclass{28.6} & \bestclass{47.8} & 13.5 & 14.9 & \highclass{47.5} & \highclass{33.0} \\
    \midrule
    \multicolumn{12}{l}{\hfill \textit{Human}} \\
    \midrule
    Human performance & $Q$, $I$ & 60.3 & 68.8 & 50.7 & 50.9 & 59.2 & 51.4 & 40.7 & 53.8 & 64.9 & 63.9 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Main results on \dataset in terms of accuracy scores. Input: $Q$: question, $I$: image, $I_c$: image caption, $I_t$: OCR texts detected from the image. ALL: overall accuracy. Question types: MC: multi-choice questions, FF: free-form questions. Mathematical reasoning types: ALG: algebraic reasoning, ARI: arithmetic reasoning, GEO: geometry reasoning, LOG: logical reasoning, NUM: numeric commonsense, SCI: scientific reasoning, STA: statistical reasoning. The highest scores among models in each section and overall are highlighted in \blue{blue} and \red{red}, respectively.}
% \vspace{-3mm}
\label{tab:scienceqa}
\end{table*}



==> backups/main_results_v2.tex <==

\begin{table*}[t!]
\centering
 \small
 \renewcommand\tabcolsep{3.0pt} % column space
 \renewcommand\arraystretch{1.0} % row space
 \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|c|c|cc|ccccccc}
    \toprule
    \header{Model} & Input & \header{ALL} & \header{MC} & \header{FF} & \header{ALG} & \header{ARI} & \header{GEO} & \header{LOG} & \header{NUM} & \header{SCI} & \header{STA}  \\ 
    \midrule
    \multicolumn{12}{l}{\hfill \textit{Heuristics  baselines}} \\
    \midrule
    % \rowcolor[rgb]{0.93,0.93,0.93} \multicolumn{11}{l}{\textit{Heuristic baselines}} \\
    Random guess & - & 17.9 & 33.1 & 0.0 & 21.7 & 14.7 & 20.1 & 13.5 & 8.3 & 17.2 & 16.3 \\
    Frequent guess & - & 26.3 & 39.6 & 10.7 & 33.1 & 18.7 & 31.4 & 24.3 & 19.4 & 32.0 & 20.9 \\
    \midrule
    % \multicolumn{11}{l}{\hfill \text{Published results (Above)} $\blacktriangle$} \\
    \multicolumn{12}{l}{\hfill \textit{Large Language Models (LLMs)} } \\
    \midrule
    Zero-shot ChatGPT~\citeyearpar{openai2022chatgpt} & $Q$ only & 23.5 & 40.6 & 3.5 & 27.7 & 15.9 & 25.7 & \highclass{21.6} & 9.9 & 41.5 & \highclass{20.5} \\
    Zero-shot GPT-4~\citeyearpar{OpenAI2023GPT4TR} & $Q$ only & 26.1 & \highclass{46.7} & 2.0 & \highclass{33.6} & 17.4 & \highclass{35.6} & 16.2 & 9.2 & \highclass{45.8} & 19.5 \\
    Zero-shot Claude-2~\citeyearpar{claude2}& $Q$ only & \highclass{26.4} & 44.4 & \highclass{5.2} & 32.8 & \highclass{20.4} & 33.3 & 13.5 & \highclass{12.1} & 36.4 & \highclass{20.5} \\
    Zero-shot ChatGPT~\citeyearpar{openai2022chatgpt} & $Q$ only & 23.5 & 40.6 & 3.5 & 27.7 & 15.9 & 25.7 & 21.6 & 9.9 & 41.5 & \highclass{20.5} \\
    Zero-shot GPT-4~\citeyearpar{OpenAI2023GPT4TR} & $Q$ only & 26.1 & 46.7 & 2.0 & 33.6 & 17.4 & 35.6 & 16.2 & 9.2 & 45.8 & 19.5 \\
    Zero-shot Claude-2~\citeyearpar{claude2}& $Q$ only & 26.4 & 44.4 & 5.2 & 32.8 & \highclass{20.4} & 33.3 & 13.5 & 12.1 & 36.4 & \highclass{20.5} \\
    \midrule
    2-shot PoT ChatGPT~\citeyearpar{openai2022chatgpt}& $Q$ only & 25.1 & 40.6 & \highclass{7.0} & 29.9 & 19.8 & 29.3 & \highclass{24.3} & \highclass{19.4} & 38.5 & 16.9 \\
    2-shot PoT GPT-4~\citeyearpar{OpenAI2023GPT4TR} & $Q$ only & 26.0 & 44.3 & 4.6 & 32.7 & 16.7 & 31.0 & \highclass{24.3} & 13.2 & \highclass{48.4} & 18.3 \\
    % \midrule
    2-shot CoT Claude-2~\citeyearpar{claude2} & $Q$ only & 24.4 & 40.6 & 5.4 & 29.2 & 19.0 & 28.0 & 5.4 & 13.9 & 36.9 & 18.9 \\
    2-shot CoT ChatGPT~\citeyearpar{openai2022chatgpt} & $Q$ only & 26.8 & 45.7 & 4.6 & 35.6 & 17.0 & 33.5 & 21.6 & 14.6 & 45.9 & 17.9 \\
    2-shot CoT GPT-4~\citeyearpar{OpenAI2023GPT4TR} & $Q$ only & \highclass{29.2} & \bestclass{50.7} & 3.9 & \highclass{41.6} & 19.3 & \highclass{41.0} & 18.9 & 13.9 & 47.5 & 18.9 \\
    \midrule
    \multicolumn{12}{l}{\hfill \textit{Augmented Large Language Models (A-LLMs)} } \\
    \midrule
    2-shot CoT Claude-2~\citeyearpar{claude2} & $Q$, $I_c$, $I_t$ & 33.2 & 44.6 & \bestclass{19.8} & 31.0 & \bestclass{32.9 }& 31.0 & 16.2 & 17.4 & 50.8 & 37.2 \\
    2-shot CoT ChatGPT~\citeyearpar{openai2022chatgpt} & $Q$, $I_c$, $I_t$ & 33.2 & 46.1 & 18.0 & 32.4 & 32.3 & 33.0 & 16.2 & 17.4 & 54.9 & 36.2 \\
    2-shot CoT GPT-4~\citeyearpar{OpenAI2023GPT4TR} & $Q$, $I_c$, $I_t$ & 33.2 & \highclass{47.2} & 16.7 & 33.5 & 30.9 & 32.2 & 13.5 & 12.5 & \bestclass{58.2} & \bestclass{37.9} \\
    % \midrule
    2-shot PoT ChatGPT~\citeyearpar{openai2022chatgpt}& $Q$, $I_c$, $I_t$ & 26.8 & 38.5 & 13.0 & 27.8 & 26.1 & 28.0 & \highclass{18.9} & 13.2 & 33.6 & 29.9 \\
    2-shot PoT GPT-4~\citeyearpar{OpenAI2023GPT4TR} & $Q$, $I_c$, $I_t$ & \highclass{33.9} & 46.3 & 19.4 & \highclass{37.4} & 31.7 & \highclass{41.0} & \highclass{18.9} & \highclass{20.1} & 44.3 & \bestclass{37.9} \\
    \midrule
    \multicolumn{12}{l}{\hfill \textit{Vision-Language Models (VLMs)}} \\
    \midrule
    IDEFICS-9B-Instruct~\citeyearpar{laurencon2023obelics} & $Q$, $I$ & 19.8 & 32.2 & 5.2 & 22.1 & 15.0 & 19.8 & 18.9 & 9.9 & 24.6 & 18.1 \\
    mPLUG-Owl-LLaMA-7B ~\citeyearpar{ye2023mplug} & $Q$, $I$ & 22.2 & 35.4 & 6.7 & 23.6 & 19.2 & 23.9 & 13.5 & 12.7 & 26.3 & 21.4 \\
    miniGPT4-LLaMA-2-7B~\citeyearpar{zhu2023minigpt} & $Q$, $I$ & 23.1 & 35.4 & 8.7 & 28.1 & 21.0 & 24.7 & 16.2 & 16.7 & 25.4 & 17.9 \\
    LLaMA-Adapter-V2-7B~\citeyearpar{gao2023llamaadapterv2} & $Q$, $I$ & 23.9 & 37.2 & 8.3 & 26.3 & 20.4 & 24.3 & \bestclass{24.3} & 13.9 & 29.5 & 18.3 \\
    InstructBLIP-Vicuna-7B~\citeyearpar{instructblip} & $Q$, $I$  & 25.3 & 37.6 & 10.9 & 21.8 & 27.1 & 20.7 & 18.9 & \bestclass{20.4} & 33.0 & 23.1 \\
    LLaVA-LLaMA-2-13B~\citeyearpar{liu2023llava} & $Q$, $I$ & 26.1 & 38.9 & 11.1 & 27.3 & 20.1 & 28.8 & \bestclass{24.3} & 18.3 & 37.3 & 25.1 \\
    Multimodal Bard~\citeyearpar{google2023bard} & $Q$, $I$  & \bestclass{34.8} & \bestclass{48.7} & \highclass{18.5} & \bestclass{46.5} & \highclass{28.6} & \bestclass{47.8} & 13.5 & 14.9 & \highclass{47.5} & \highclass{33.0} \\
    \midrule
    \multicolumn{12}{l}{\hfill \textit{Human}} \\
    \midrule
    Human performance & $Q$, $I$ & 60.3 & 68.8 & 50.7 & 50.9 & 59.2 & 51.4 & 40.7 & 53.8 & 64.9 & 63.9 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Main results on \dataset in terms of accuracy scores. Input: $Q$: question, $I$: image, $I_c$: image caption, $I_t$: OCR texts detected from the image. ALL: overall accuracy. Question types: MC: multi-choice questions, FF: free-form questions. Mathematical reasoning types: ALG: algebraic reasoning, ARI: arithmetic reasoning, GEO: geometry reasoning, LOG: logical reasoning, NUM: numeric commonsense, SCI: scientific reasoning, STA: statistical reasoning. The highest scores among models in each section and overall are highlighted in \blue{blue} and \red{red}, respectively.}
% \vspace{-3mm}
\label{tab:scienceqa}
\end{table*}



==> backups/our_dataset_examples.tex <==
% TabMWP - Knowledge Retrieval 
\begin{table*}[th!]
\centering
\fontsize{10.0pt}{\baselineskip}\selectfont
%\linespread{0.99}\selectfont
\begin{boxedminipage}{1.0\columnwidth}

% Instruction
\mybox{\centering$\triangleright$ \textit{Instruction}}

Read the following table and question, and generate the domain-specific knowledge as the context information that could be helpful for answering the question.

% In-context example
\mybox{\centering$\triangleright$ \textit{In-context example(s)}}

\textbf{Table:}\\
adsaf

\textbf{Question:} The table shows a function. Is the function linear or nonlinear?\\

\textbf{Knowledge:}\\
- A linear function is a function whose graph is a straight line.\\
- A nonlinear function is a function whose graph is not a straight line.\\
- The equation of a linear function is $y = mx + b$, where $m$ is the slope and $b$ is the $y$-intercept.\\
- The equation of a nonlinear function is not $y = mx + b$.

\end{boxedminipage}
\caption{The prompt constructed for the ``Knowledge Retrieval'' module on the task.}
\label{fig:planner_tabmwp_kr}
\end{table*}

==> backups/our_new_3_dataset.tex <==


\begin{table*}[ht!]
\centering
\fontsize{10.0pt}{\baselineskip}\selectfont
\linespread{1.0}\selectfont

\begin{boxedminipage}{0.32\columnwidth}
\textbf{Answer Generator (Prediction):} 
\red{(B) yellow} \\
\textbf{Correct Answer (Ground Truth):} 
\end{boxedminipage}
 \hfill
\begin{boxedminipage}{0.33\columnwidth}
\textbf{Answer Generator (Prediction):} 
\red{(B) yellow} \\
\textbf{Correct Answer (Ground Truth):} 
\end{boxedminipage}
 \hfill
\begin{boxedminipage}{0.33\columnwidth}
\textbf{Answer Generator (Prediction):} 
\red{(B) yellow} \\
\textbf{Correct Answer (Ground Truth):} 
\end{boxedminipage}

\caption{An example captioning model in providing an accurate textual description of the given visual context.}
\label{fig:failure_scienceqa_2}
\end{table*}

==> contents/app_gpt4v_abstain.tex <==
\clearpage
\subsection{Abstaining from Responding}
\label{sec:gpt4v_abstain}

We observed that both Multimodal Bard and GPT-4 often abstain from responding.  Specifically, Multimodal Bard returns ``Sorry, I can't answer this question'' (7.0\%) or ``I can't process this file'' (0.8\%), while GPT-4V responds with ``Sorry, I cannot help with that.'' (7.0\%). As illustrated in Figures \ref{fig:example_699} through \ref{fig:example_more_safety}, these patterns can be attributed
to patterns in large language models that have been characterized
as ``exaggerated safety behaviors'' \citep{rottger2023xstest}. 
%to \textit{exaggerated safety behaviors}, which are also observed %in large language models \citep{rottger2023xstest}. 
Further research is necessary to explore these behaviors in large multimodal models.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[th!]
\fontsize{9.0pt}{\baselineskip}\selectfont
\linespread{0.9}\selectfont
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\begin{minipage}[s][2.8cm]{0.35\columnwidth}
\includegraphics[height=2.8cm]{images/safety/699.jpg}
\end{minipage}
\hspace{1mm}
\begin{minipage}[s][2.8cm]{0.6\columnwidth}
\textbf{ID:} 699\\\\
\textbf{Question:} What is the age gap between the center and the rightmost person? (unit: years) \\\\
\textbf{Ground truth:} \textbf{\green{0}} \\\\
\end{minipage}
\end{mybody}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{mybody}
% \textbf{LLaMA-Adapter-V2:}
% \red{The age gap between the center and the rightmost person is 1 year.}
% \end{mybody}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{mybody}
% \textbf{LLaVA:} 
% \red{The center person is 24 years old, and the rightmost person is 19 years old, which means there is a 5-year age gap between them.}
% \end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\textbf{Multimodal Bard:} \red{Sorry, I can't help with images of people yet.}
\end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\textbf{GPT-4V:} \red{Sorry, I cannot help with that.} 
\end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\captionof{figure}{The example where both Multimodal Bard and GPT-4V refuse to respond to the question involving the age information of two famous soccer players.}
\label{fig:example_699}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[th!]
\fontsize{9.0pt}{\baselineskip}\selectfont
\linespread{0.9}\selectfont
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\begin{minipage}[s][2.8cm]{0.27\columnwidth}
\includegraphics[height=2.8cm]{images/safety/740.jpg}
\end{minipage}
\hspace{1mm}
\begin{minipage}[s][2.8cm]{0.70\columnwidth}
\textbf{ID:} 740\\\\
\textbf{Question:} What percent of the stands are full? \\\\
\textbf{Choices:} (A) 15 (B) 100 (C) 50  \\\\
\textbf{Ground truth:} \textbf{\green{(A) 15}}
% \textbf{Solution:} text
\end{minipage}
\end{mybody}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{mybody}
% \textbf{LLaMA-Adapter-V2:}
% \red{The correct answer is (D) 50. The stands are half full, with approximately half of the seats occupied.}
% \end{mybody}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{mybody}
% \textbf{LLaVA:} \red{The stands are 100\% full, meaning that all available seats are occupied by spectators.}
% \end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\textbf{Multimodal Bard:} \red{Sorry, I can't help with images of people yet.}
\end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\textbf{GPT-4V:} \red{Sorry, I cannot help with that.} 
\end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\captionof{figure}{While the question seeks an estimate of the number of people in the stands, both Multimodal Bard and GPT-4V opt not to provide responses.}
\label{fig:example_740}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[th!]
\fontsize{9.0pt}{\baselineskip}\selectfont
\linespread{0.9}\selectfont
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\begin{minipage}[s][2.8cm]{0.24\columnwidth}
\includegraphics[height=2.8cm]{images/safety/779.jpg}
\end{minipage}
\hspace{1mm}
\begin{minipage}[s][2.8cm]{0.73\columnwidth}
\textbf{ID:} 779\\\\
\textbf{Question:} Is the cardiac silhouette less than half the diameter of the diaphragm? \\\\
\textbf{Choices:} (A) Yes (B) No \\\\
\textbf{Ground truth:} \textbf{\green{(A) Yes}} \\\\
% \textbf{Solution:} text
\end{minipage}
\end{mybody}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{mybody}
% \textbf{LLaMA-Adapter-V2:} \red{No, the cardiac silhouette is not less than half the diameter of the diaphragm.}
% \end{mybody}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{mybody}
% \textbf{LLaVA:} The cardiac silhouette is less than half the diameter of the diaphragm.
% \end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\textbf{Multimodal Bard:} \red{I can't process this file.}
\end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\textbf{GPT-4V:} \red{Sorry, I cannot help with that.} 
\end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\captionof{figure}{An instance where both Multimodal Bard and GPT-4V do not address a question within the medical domain.}
\vspace{-1mm}
\label{fig:example_779}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[th!]
\fontsize{9.0pt}{\baselineskip}\selectfont
\linespread{0.9}\selectfont
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\begin{minipage}[s][5.0cm]{0.26\columnwidth}
\includegraphics[height=5.0cm]{images/safety/821.jpg}
\end{minipage}
\hspace{1mm}
\begin{minipage}[s][5.0cm]{0.71\columnwidth}
\textbf{ID:} 821\\\\
\textbf{Question:} Are most of the people young men? \\\\
\textbf{Choices:} (A) Yes (B) No \\\\
\textbf{Ground truth:} \textbf{\green{(A) Yes}} \\\\
% \textbf{Solution:} text
\end{minipage}
\end{mybody}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{mybody}
% \textbf{LLaMA-Adapter-V2:} \red{No, most of the people in the image are not young men. There are both young men and women present in the scene.}
% \end{mybody}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{mybody}
% \textbf{LLaVA:} The correct answer is A, Yes. Most of the people in the image are young men.
% \end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\textbf{Multimodal Bard:} \red{Sorry, I can't help with images of people yet.}
\end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\textbf{GPT-4V:} \red{Sorry, I cannot help with that.} 
\end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\captionof{figure}{In this example related to the age and gender of a group of people, both Multimodal Bard and GPT-4V choose not to respond.}
\label{fig:example_821}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[th!]
\fontsize{9.0pt}{\baselineskip}\selectfont
\linespread{0.9}\selectfont
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\begin{minipage}[s][3.8cm]{0.37\columnwidth}
\includegraphics[height=3.8cm]{images/safety/352.jpg}
\end{minipage}
\hspace{1mm}
\begin{minipage}[s][3.8cm]{0.63\columnwidth}
\textbf{ID:} 352\\\\
\textbf{Question:} How many people will fit in the smaller vehicle? \\\\
\textbf{Ground truth:} \textbf{\green{1}} \\\\
% \textbf{Solution:} text
\end{minipage}
\end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\begin{minipage}[s][5.0cm]{0.26\columnwidth}
\includegraphics[height=5.0cm]{images/safety/516.jpg}
\end{minipage}
\hspace{1mm}
\begin{minipage}[s][5.0cm]{0.71\columnwidth}
\textbf{ID:} 516\\\\
\textbf{Question:} Are most the stepping stones square?\\\\
\textbf{Choices:} (A) Yes (B) No \\\\
\textbf{Ground truth:} \textbf{\green{(B) No}} \\\\
% \textbf{Solution:} text
\end{minipage}
\end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{mybody}
\textbf{GPT-4V:} \red{Sorry, I cannot help with that.} 
\end{mybody}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\captionof{figure}{Two additional examples where GPT-4V does not respond for unspecified reasons.}
\label{fig:example_more_safety}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> contents/app_gpt4v_future.tex <==
\clearpage
\subsection{Future Directions}
\label{sec:gpt4v_future}

Text


\red{
As illustrated in \S \ref{sec:model_comparison}, GPT-4V accurately predicts the correct answer for the logical reasoning question present in Figure \ref{fig:example_852}, while all other LMM and LLM baselines fail. GPT-4V also provides an accurate prediction for the example in Figure \ref{fig:example_824}, which requires table perception, statistical reasoning, and arithmetic reasoning. However, GPT-4V fails to answer the fundamental statistical question in Figure \ref{fig:example_852} and cannot resolve the linguistic ambiguity using visual cues in Figure \ref{fig:example_458_llm}. Additional examples are provided in \S \ref{sec:experiments_gpt4v}.
}


% \subsection{Hallucinations}
% \label{sec:gpt4v_hallucination}

% 10+ examples in the appendix 


